Alternative Paths Planner (APP) for Provably Fixed-time Manipulation Planning in Semi-structured Environments

In many applications, including logistics and manufacturing, robot manipulators operate in semi-structured environments alongside humans or other robots. These environments are largely static, but they may contain some movable obstacles that the robot must avoid. Manipulation tasks in these applications are often highly repetitive, but require fast and reliable motion planning capabilities, often under strict time constraints. Existing preprocessing-based approaches are beneficial when the environments are highly-structured, but their performance degrades in the presence of movable obstacles, since these are not modelled a priori. We propose a novel preprocessing-based method called Alternative Paths Planner (APP) that provides provably fixed-time planning guarantees in semi-structured environments. APP plans a set of alternative paths offline such that, for any configuration of the movable obstacles, at least one of the paths from this set is collision-free. During online execution, a collision-free path can be looked up efficiently within a few microseconds. We evaluate APP on a 7 DoF robot arm in semi-structured domains of varying complexity and demonstrate that APP is several orders of magnitude faster than state-of-the-art motion planners for each domain. We further validate this approach with real-time experiments on a robotic manipulator.

==> 02introduction.tex <==
%% motivate the need of planners for semi-static environments
In a wide range of environments, be it warehouses, factories or homes, robots share their workspace with humans or other robots. While the obstacle occupancy in such environments is largely fixed or static, yet small regions within these environments may vary in occupancy during operation. We categorise such environments as \emph{semi-structured}. Additionally in these applications robots are often performing repetitive tasks and require fast and reliable motion planning capabilities.

%% use example
Consider the scenario in Fig.~\ref{fig:cover}. The robot must grasp the bowl while avoiding the pitchers, table and walls.
%Most of the environment (e.g. table, walls, free space above the table etc.) can be assumed to be known, and since the task of picking up an object from a tabletop is repetitive, some information from previous similar planning queries can be re-used to speedup planning.
Most of the environment (e.g. table, walls, free space above the table etc.) can be assumed to be known, and since the task is repetitive some information from previous planning queries can be re-used to speedup planning.
 %More commonly used planning algorithms such as RRTs neither exploit the distinction between static and movable obstacles, nor do they take advantage of the repetitive nature of planning problems to speedup planning. 
Commonly used algorithms such as RRTs~\cite{kuffner2000rrt} neither exploit the distinction between static and movable obstacles nor take advantage of the repetitive nature of planning problems to speedup planning. 

%% existing approaches
%Preprocessing based methods like PRMs, precompute roadmaps to speedup online planning. They
Roadmap-based methods like PRMs are either limited to fully static environments or incur considerable overheads in repair operations which they require to handle movable obstacles. While there exists several algorithms that use information from previous similar planning episodes such as Lightning~\cite{berenson2012robot}, E-graphs~\cite{Phillips-RSS-12} etc., their performance also degrades when the past information is invalidated by the changes in the environment. All these methods therefore can not provide fixed-time planning guarantees. 

%% my prior work
Recently, provably fixed-time motion planning approaches have been proposed for repetitive tasks in fully known environments~\cite{islam2019provable},~\cite{islam2020provably}. They precompute library of paths using the known models of obstacles and other task-specific information. These approaches have been used before for mail-sorting~\cite{islam2019provable} and for grasping objects moving down a conveyor belt~\cite{islam2020provably}. They, however, are also not designed to handle movable obstacles.

\begin{figure}[bt]
\centering
\includegraphics[width=0.8\columnwidth]{figs/cover.jpg}
\caption{Semi-structured tabletop manipulation scenario --- The robot must grasp the bowl while avoiding pitchers and the table itself; the pitchers and bowl may be at any position. The Alternate Paths Planner (APP) guarantees to find solution for any configuration within few microseconds.}
\label{fig:cover}
\vskip -0.5cm
\end{figure}

%% our contribution
%In this work we aim to extend these recent approaches to be able to handle movable obstacles while still provably fixed-time planning guarantees.
In this work we extend these approaches to handle movable obstacles while still guaranteeing provably fixed-time planning.
%key idea of our approach is to generate multiple alternative paths for each planning problem, such that for any configuration of movable obstacles, one of these alternative paths is guaranteed to be traversable.
The key idea is to generate multiple alternative paths for each planning problem, such that for any configuration of movable obstacles, one path is guaranteed to be traversable.
One approach to achieve this is to enforce %a constraint
that these paths are \emph{disjoint}: they are separated enough that no single obstacle configuration can intersect two paths simultaneously.
To get the aforementioned guarantee, $n$ movable obstacles require generating only $n+1$ fully disjoint paths.
%However, if $n+1$ disjoint paths cannot be found for the given problem, our approach uses more preprocessing and finds additional paths to provide the guarantee.
However, if $n+1$ disjoint paths cannot be found for the given problem, we find additional additional paths partially-overlapping paths to provide the same guarantee.
%We make some simplistic assumptions about the geometry of movable obstacles to provide strong guarantees on the planning time.
We call this approach \emph{Alternative Paths Planner (APP)}

%APP can be applied to many performance critical real-world robotics use cases such as mail-sorting, conveyor-belt picking, and shelving. 
APP can be applied to performance-critical real-world use cases such as mail-sorting, conveyor-belt picking, and shelving. 
For scenarios with multiple movable obstacles, we demonstrate microsecond-scale lookup times and achieve a 100\% success rate. We include experimental results from three domains, compare with state-of-the-art existing approaches and validate our approach with a real-world case study. 

\begin{comment}
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In the real world, robots are often employed in static environments with few moving obstacles doing highly repetitive tasks.
For practical applications, robots are often doing highly repetitive tasks in static environments with few moving obstacles.
%Nevertheless, few existing motion planners 
Few existing motion planners, however, take advantage of this fact. 
%Motion planners from sampling-based algorithms like Rapidly-Exploring Random Trees (RRT)~\cite{kuffner2000rrt} or LazyPRM~\cite{kavraki2000path} to search-based planning algorithms like ARA*~\cite{likhachev2004ara} 
Sampling-based planning algorithms (e.g., Rapidly-Exploring Random Trees (RRT)~\cite{kuffner2000rrt}, LazyPRM~\cite{kavraki2000path}) and search-based (e.g., ARA*~\cite{likhachev2004ara}) planning algorithms are generally designed to function in unseen environments where minimal information can be re-used from one plan to the next. Conversely, preprocessing-based planning approaches cannot deal with obstacles that may be at unknown positions~\cite{islam2019provable,islam2020provably}.

Consider Fig.~\ref{fig:cover}. The robot must grasp the bowl while avoiding the pitchers, table, and walls.
Most of the environment can be assumed to be known, and some information from previous planning queries can be re-used over and over again. 
%Certain planners do take advantage of information from previous attempts, like Lightning~\cite{berenson2012robot}, E-graphs~\cite{Phillips-RSS-12}, or LazyPRM~\cite{kavraki2000path}, but these often run into issues when that past information is made invalid and can have very sub-optimal performance.
While planners such as Lightning~\cite{berenson2012robot}, E-graphs~\cite{Phillips-RSS-12}, and LazyPRM~\cite{kavraki2000path} do take advantage of information from previous attempts, these planners tend to perform sub-optimally when past information is made invalid due to changes in the environment.

Another approach is to explicitly pre-process the environment based on known geometry and some information about what potential goals may appear at runtime. This approach has been used before for mail-sorting~\cite{islam2019provable} and for handling objects moving down a conveyor belt~\cite{islam2020provably}. Preprocessing allows us to amortize the cost of future queries by doing most of the work for a particular environment ahead of time, meaning that at run-time trajectories can be found in microseconds. 
%However, preprocessing methods by their very nature cannot handle moving obstacles.
Conventional preprocessing methods, however, are not designed to handle movable obstacles.

%Most human environments - including but not limited to the sorts of logistics and manufacturing settings where we often see robots employed - are semi-structured. While they have static components as assumed by prior work~\cite{islam2019provable,islam2020provably}, they also have a number of obstacles that may appear in different locations. These could be objects deposited by another robot, moved by a human, or could in fact be a human that might be reaching into the robot's workspace.

\begin{figure}[bt]
\centering
\includegraphics[width=\columnwidth]{figs/fi-realrobot.jpg}
\caption{Semi-structured tabletop manipulation scenario. The robot must grasp the bowl while avoiding mugs and the table itself; the mugs and bowl may be at any position. The Alternate Paths Planner (APP) guarantees solutions in this scenario.}
\label{fig:cover}
\end{figure}

How can we extend preprocessing-based approaches in such a way that we can guarantee extremely fast motion planning in the presence of obstacles with unknown configurations? One solution is to enforce the constraint that our planner will generate multiple paths for each possible goal, such that if some paths are blocked we can fall back to a different option. This requires designing an algorithm that will produce not just multiple paths but multiple \textit{disjoint} paths in order to guarantee that a path will be viable regardless of obstacle configuration. We define paths as \textit{disjoint} if they do not intersect at any point along their trajectories \textit{and} there are no possible obstacle configurations that would collide with both paths. A set of fully disjoint paths would allow us to handle up to $n$ obstacles with unknown positions by creating $n+1$ paths.
%, paths that do not intersect at any point along their trajectory in order to guarantee that a path will be viable regardless of obstacle positions. This would allow us to handle up to $n$ obstacles with unknown positions by creating $n+1$ paths.

%However, there's a problem: in many scenarios, 
For many practical scenarios, however, we cannot compute $n+1$ completely disjoint paths. Instead, we must find a set of trajectories such that there always exists at least $n+1$ disjoint paths for each segment of a trajectory.
%, which we do via a recursive algorithm that will break down trajectories into multiple parts and solving for disjoint paths multiple times. 
We use a recursive algorithm to split trajectories into smaller segments, solving for disjoint paths at each level.
%The result is a set of trajectories 
The resulting set of trajectories is guaranteed to include solutions that will avoid up to $n$ obstacles for a given goal region. We call this approach the \textit{Alternate Paths Planner~(APP)}.

APP can be applied to many different real-world robotics use cases such as mail-sorting, conveyor belt picking, sorting, and shelving. 
%We see  microsecond level lookup times and high success rates for scenarios with multiple moving obstacles, compared to a wide variety of commonly-used and state-of-the-art motion planners. We show results in three domains, plus describe a real-world case study.
For scenarios with multiple movable obstacles, we demonstrate microsecond-scale lookup times and achieve success rates much higher than a wide variety of commonly-used and state-of-the-art motion planners. We include simulated results from three domains and further validate our approach with a real-world case study. 

%The primary contributions of this work are:
%\begin{itemize}
%    \item the Alternative Paths Planner for guaranteed-time task and motion planning in semi-structured environments
% to find \end{itemize}
\end{comment}

==> 03background.tex <==
% Sampling-based motion planning provides very fast feasible solutions, but sacrifices optimality. RRT-Connect~\cite{kuffner2000rrt} has been widely used and modified, and is still an extremely fast and reliable approach. Lighting~\cite{berenson2012robot} builds on RRT-Connect, but with reuse of trajectories.
% (BIT)~\cite{gammell2020batch}
% InformedRRTstar~\cite{gammell2018informed}
% RRTstar~\cite{karaman2011sampling}
%RLDS -- re-use task structure with known low-level policies~\cite{paxton2019representing}
%\subsection{Preprocessing-based Planning}

%% Preprocessing-based methods
Preprocessing-based motion planners often prove beneficial for real-time planning.
They analyze the configuration space offline to generate an approximate representation of the planning problem, that can be exploited online to speed up planning.
The Probablistic Roadmap Method (PRM)~\cite{kavraki1996probabilistic} is a classical instance of such a preprocessing-based planner.
It precomputes a graph of the collision-free C-space and answers any query by connecting the start and goal configurations to this roadmap, followed by a graph search.
A variety of techniques to improve the PRM have been introduced over the years: minimizing expensive collision checks~\cite{kavraki2000path}, accounting for dynamic environments~\cite{leven2002framework,yang2017hdrm}, and capturing repetitive motions~\cite{lehner2018repetition}.
Although PRMs are fast to query their computational complexity depends on the underlying approximation. Moreover, in the case of movable objects, they would require edge re-evaluation which is often computationally expensive.

%% Experience based planners
Instead of preprocessing collision information offline, another class of planners exploits previous experiences to speed up search~\cite{Phillips-RSS-12,berenson2012robot,coleman2015experience}. 
Experience graphs~\cite{Phillips-RSS-12} provide speed up in planning times for repetitive tasks by trying to reuse previous planning queries.
These methods are also augmented with sparsification techniques~\cite{dobson2014sparse,salzman2014sparsification} to reduce the memory footprint of the resulting roadmap.
The P-CAP method~\cite{zhang2018p} relates to our approach.
It pre-computes a dense set of alternative paths that enables aerial vehicles to deal with obstacles and successfully navigate unstructured environments.
Nevertheless, none of the mentioned algorithms provide fixed
planning-time guarantees that we strive for in our application.


%% Fixed time planners
Provably fixed-time planners were recently proposed
in~\cite{islam2019provable,islam2020provably} for applications that involve repetitive tasks. Given a start state and a goal region, they precompute a compressed set of paths that can be utilized online to plan to any goal within the goal region in constant or bounded time.
While our approach APP draws inspiration from these works we focus on enabling online obstacle avoidance by explicitly accounting for movable obstacles during the preprocessing phase by using the alternative paths planning approach.
Finally in the context of fixed-time planning, there is a family of real-time planners from the search-based planning community (see, e.g.,~\cite{KL06,KS09,korf1990real}). To provide guarantees on planning time the search only looks at a finite horizon, generating a partial plan, and interleaves
planning and execution. Moreover they are only limited to low-dimensional planning problems (2D,3D).


==> 12introduction-old.tex <==
High level idea: pre-process environment to generate a roadmap of different "regions" within which our robust low-level policies (perhaps RMPs) are guaranteed to work.

Eventually we could learn heuristics or policies to accompany this -- since the quality of the low-level policy should determine the roadmap this will presumably make things easier.

Comparisons can be made to the codebase from~\cite{garrett2019online}, which will be much slower. We probably do not want to handle partial observability at least to begin with, but that doesn't necessarily mean it's a big issue yet.

\textbf{Task planning robustness}: given some set of possible disruptions (e.g. closed drawers, dropped objects), compute a directed acyclic graph to the goal. Once we do this, if one of these disruptions occurs, no replanning is necessary.

\textbf{Time-aware subregion computation}: some subregions aren't connected until we arrive at certain logical states (e.g. a drawer is open). When a subregion contains something moveable like a drawer, it may need to be broken up into multiple subregions. We recompute subregions locally whenever a subregion is effected by a moving obstacle (like an opening drawer).

Goals:
\begin{itemize}
    \item Within some bounded factor $\lambda$ of the length of a discrete task plan $P$, ensure that we can always arrive at a plan (or determine that such a plan is impossible.
    \item Once given our task plan, we can recover immediately so long as the disturbance is within the space of the original task plan (subsumes RLDS~\cite{paxton2019representing})
    
\end{itemize}

==> back.tex <==

Specifically we are interested in pick and place manipulation tasks (PPM).

We are assuming:
\begin{itemize}
    \item task planning domain is given with high-level actions describing manipulations of the world (can be in PDDL, STRIPS, whatever we want).
    \item domain includes region preconditions, e.g. for grasping an object or a handle. Can be a sampler, as in previous work~\cite{garrett2019online}
    \item model of the environment, e.g. the kitchen 
    \item object models?  Maybe we can weaken this assumption later and use less specific object models (e.g. other mugs, grab an out-of-distribution mug)
\end{itemize}

Task planning graph is over semantics and actions; we need to add a decomposition over reachability regions/affordances that allow us to do certain fixed actions like opening doors or picking up objects.

\subsection{Task Graph}

Build a graph over sub-regions in the given environment. We need to determine what the relationship is between the (discrete, symbolic) task graph and the real world.

Goal sub-regions associated with the end points of each high-level action. Maintain connectivity (plus number of disjoint paths) between goal regions, where these are pre-conditions for various high level actions/primitives:
\begin{itemize}
    \item grasp an object or handle
    \item place on a surface
    \item move arm
    \item move a drawer/door (to open it or close it) -- listed separately because it has to be linear, and has a separate policy.
    \item release an object/gripper
    \item move base (if we have a mobile robot)
\end{itemize}

These include (constrained) action regions. These are things like the linear motion to open a drawer or move from pre-grasp to grasp position. These are a part of the big ``task graph'' that we need to search over.

Each symbolic state induces some configuration space that we can search in.

\subsection{Computing Subregions}

\textbf{This section is probably not right; see details below.}

Start with a goal-sampler. Goal is to find a region which will allow us to locally move to all of the different subgoals.

We could split subgoal accessibility regions later on into multiple regions, if we have different disjoint groups of subogals (i.e. not all subgoals can be reached).

Computing the minimal number of subregions would be great. 

Subregion creation could be done in parallel (using Isaac Gym for example). Create many different environments, seed positions and build out interconnected regions where we can use these.

\subsection{Computing the Connectivity Graph}

Parallelization of subregion connectivity graph: compute reachability from each subregion to the others, (sparse) transition matrix between subregions where connecting path is computed via some motion planner (e.g. RRT).

We could use some good low-level policy, e.g. RMPs, for moving within regions -- or using RRT plan.

We use some trajectory primitives (spline or DMPs) to connect sub-regions. Maybe we could just use a planner instead?

\subsection{Example Task}

Two example tasks:
\begin{itemize}
    \item kitchen domain: going into cabinets; retrieve object(s) from cabinets
    \item tabletop manipulation: re-arrange things on the cart.
    \item kitting: moving objects into bins, potentially with lids or other coverings (so we have to move something out of the way, and so that we have this ``task graph'' to execute)
\end{itemize}

Goal samplers: surfaces we can place objects on, handles to grasp, and object grasp poses.





\newpage
\section{Algorithmic Framework}

\subsection{Problem Setup and Assumptions}
\label{subsec:setup}
Let \calX be the configuration space of the robot. Let $\Sstart \in \calX$ be a fixed start configuration of the robot and \calG be the goal region. \calG could be defined in the configuration space \calX i.e $\calG \subset \calX$ or it could be under-defined for higher dimensional planning problems e.g. as the position~$(x,y,z)$ or pose~$(x,y,z, roll, pitch,yaw)$ of a target object or the robot end-effector. \calG is discretized to have a finite set of goals $G$. 

Let \calW be a semi-static world in which the robot operates. \calW contains a fixed set of movable obstacles $\calO = \{o_1, o_2, o_3,...,o_n\} \in \calW$ which could be displaced in between different planning queries. Additionally, \calW has a partial occupancy which is static i.e $\calW_S = \calW \backslash \calO$. The motion planning problem is to find a collision-free path for the robot operating in \calW from \Sstart to any goal $g \in G$.

\begin{assumption}
We approximate the geometry of all obstacles $o \in \calO$ by the same shape e.g a sphere of radius $r$ if \calW is a 3D world (or a  circle if \calW is 2D).
\end{assumption}

\subsection{Approach}
In this work, we aim to develop an algorithm that can provide provable bounds on the planning time for each planning query. Furthermore we want the bounds to be small to guarantee real-time performance. Before we describe our approach, we begin by briefly describing a strawman algorithm which solves the aforementioned problem with the provable bounded-time guarantee but is practically prohibitive to use because of its memory and computational requirements. This will also prepare the ground to describe our method which also provides bounded-time guarantee but with minimal memory and computational load.


\subsubsection{Strawman Algorithm}
Let's assume that we have access to a conventional motion planner \calP that can be used offline to find feasible paths to a given planning problem. The naive approach of providing bounded-time guarantees is to precompute and store paths for all possible planning problems using \calP owing to the problem setup described in Sec.~\ref{subsec:setup}, offline in a preprocessing stage, and at query time use a hash lookup table to answer any query in bounded time. Specifically, it requires computing the lookup table
$$
\calM : G \times \textrm{Pos}(o_1) \times \textrm{Pos}(o_2) \times ... \times \textrm{Pos}(o_n) \rightarrow \{\pi_1, \pi_2,\pi_3,...\}
$$

\noindent where $\textrm{Pos}(o_i) \subset \calW$ constitutes the set of all possible positions that object $o_i$ can attain. The lookup table thus maps every combination of goal and positioning of all the $n$ obstacles to a unique path resulting in $|G|.|\textrm{Pos}(o_1)|.|\textrm{Pos}(o_2)|....|\textrm{Pos}(o_n)|$ paths. Assuming that each object $o_i$ can acquire the same set of positions in $\calW$, the space complexity then is $O(|G|.n^{\textrm{Pos}(o_i)})$ which is exponential in the number of movable objects in \calO. This complexity clearly is severely restrictive in practice.

\subsubsection{Proposed Approach}
While the strawman algorithm provides bounded-time guarantees, its memory and precomputation load is prohibitive for practical purposes. To this end we propose an algorithm that can provide bounded-time guarantees but requiring significantly smaller resources in practice.

Our key idea is that, for the given \Sstart and $g$, instead of precomputing path for every possible positioning of obstacles \calO, our algorithm systematically precomputes a small set of paths from \Sstart to $g$ with the guarantee that for any possible positioning of the \calO in \calW, at least one of the paths from this set will be collision free. At query time, this path can be looked up efficiently in provably bounded time.

\subsubsection{Algorithm Overview}
Before we describe the approach, we introduce some terminology.

\begin{definition}[Envelope]
For a path $\pi$, an envelope $e_\pi \subset Pos(o_1) \cup Pos(o_3) \cup...\cup Pos(o_n)$ is a set of all obstacle positions of any $o \in \calO$ that collides with it.
\end{definition}

\begin{definition}[Disjoint paths]
\label{def:disjointness}
A set of paths $\{\pi_1,\pi_2,...\}$ are disjoint if their corresponding envelopes $\{e_{\pi_1},e_{\pi_2},...\}$ are non-overlapping sets.
\end{definition}

For simplicity, consider a simple planning problem of finding a collision-free path from \Sstart to a goal $g \in G$ in the presence of a single movable obstacle $o$ and some static occupancy $\calW_S$ as depicted in Fig. We first find a path $\pi_1$ from \Sstart to $g$ using \calP while avoiding collisions with only $\calW_S$. Next we construct an envelope $e_{\pi_1}$ around $\pi_1$. We then attempt to find a second path $\pi_2$ that avoids collisions with $\calW_S$ as well as with $e_{\pi_1}$. This gives us two disjoint paths $\pi_1$ and $\pi_2$ (since $e_{\pi_2}$ would not overlap with $e_{\pi_1}$ by Def.~\ref{def:disjointness}). These two paths constitute the minimal set of paths with the guarantee that for any positioning of $o \in \calW$, one of these two paths will be collision free. At query time given any position of $o$, we can check if it lies within $e_{\pi_1}$ or not and use the path $\pi_2$ or $\pi_1$ respectively. If we store envelopes as hashtables, we can perform this check in constant or bounded time (add citation).

\textbf{Extending to $n$ movable obstacles:} A single movable obstacle, requires two disjoint paths. Extending to $n$ objects would require $n+1$ disjoint paths. Therefore, for the scenarios in which $n+1$ disjoint paths exists and \calP can find them within a given allowed planning time, the computational complexity of the preprocessing phase grows linearly with number of movable obstacles i.e $O(|\calO|)$. However, if the \calP fails to find $n+1$ disjoint paths, then the algorithm requires more preprocessing efforts to find more paths such that the criterion that for any possible positioning of the set of obstacles \calO, at least one of the paths from the set is guaranteed to be collision free, is satisied. The details of the complete preprocessing and query algorithms are discussed in the following section.

\subsection{Algorithm Details}
We now describe the two phases of our algorithm i.e. the preprocessing and the query phases.

\subsubsection{Preprocessing}
The preprocessing algorithm is described in Alg.~\ref{alg1}. It starts with finding the first collision free path $\pi_1$ from \Sstart to the given goal $g \in G$ in $\calW_S$. For each computed path $\pi_j$, the algorithm maintains the set of envelopes $\calE_{\pi_j}$ that were avoided while computing $\pi_j$. For the first path $\pi_1$, the set $\calE_{\pi_1}$ is empty since \calP only considers $\calW_S$ for this step. The algorithm then runs a loop for N=$|\calO|$ iterations, attempting to find N more mutually disjoint paths (loop at line~\ref{alg1:l1}). Another loop at line~\ref{alg1:l2} is needed for the case when $N+1$ disjoint paths do not exist and therefore, more than one paths are computed in a single iteration of loop at line~\ref{alg1:l1}.
In every iteration of the loop at line~\ref{alg1:l2}, the algorithm first constructs the envelope $e_{\pi_j}$ around the path $\pi_j$ found in the previous iteration of loop at line~\ref{alg1:l1}. Next, $\pi_j'$ is computed while avoiding collisions with $\calE_{\pi_j}'$ which is the union of $e_{\pi_j}$ and the envelopes in $\calE_{\pi_j}$. $\calE_{\pi_j}'$ thus constitutes the set of avoided envelopes for $\pi_j'.$

For the case when \calP fails to find the disjoint path at any iteration of loop at line~\ref{alg1:l1}, the algorithm bisects one of the envelopes (line~\ref{alg1:bisect} and Alg.~\ref{alg2}) that \calP attempted to avoid, resulting in two sets of envelopes (each one containing a bisected envelope along with the remaining envelopes). \calP then tries to find paths around the envelopes in each of the two sets independently. Note that this process (Alg.~\ref{alg2}) repeats recursively until either \calP successfully finds paths around all the newly created sets of envelopes or until further recursion is not possible. The latter occurs in the worst case, when the algorithm recurses down to the deepest level, where each envelope contains individual obstacle positions. Owing to the structure of these envelopes, we implement them as binary-trees. Because of this envelope bisection, the algorithm may compute more than one paths in a single iteration of loop at line~\ref{alg1:l1}. It therefore maintains a set of paths $\Pi_i$ for each iteration and attempts to compute disjoint paths for each $\pi_j \in \Pi_i$ in the next iteration.

\begin{algorithm}[t]
\caption{\textsc{Preprocess($g$)}} \label{alg1}
\AlgFontSize
\hspace*{\algorithmicindent} \textbf{Inputs:} $\Sstart, \calW_S, \calO$
\begin{algorithmic}[1]
\State $\pi_1 \leftarrow$ \textsc{FindPath}($\Sstart,g,\calW_S$)
\State $\calE_{\pi_1} \leftarrow \emptyset$
\State \textsc{SetAvoidedEnvelopesOfPath($\pi_1,\calE_{\pi_1}$)}
\State $\Pi_1 \leftarrow \pi_1$
% \State $\calE \leftarrow \emptyset$
\For {i = 1 to N}  \Comment{N = $|\calO|$}  \label{alg1:l1}
    \State $\Pi_{i+1} \leftarrow \emptyset$
    \For{each $\pi_j \in \Pi_i$} \label{alg1:l2}
    \State $e_{\pi_j} \leftarrow$ \textsc{ConstructEnvelope($\pi_j$)}
    % \State $\calE \leftarrow \calE \cup \{e\}$
    % \State $\Pi_{i+1} \leftarrow$ 
    % \For{each $e \in \calE_i$}
        \State $\calE_{\pi_j} \leftarrow$ \textsc{GetAvoidedEnvelopesOfPath}($\pi_j$)
        \State $\calE_{\pi_j'} \leftarrow \calE_{\pi_j} \cup \{e_{\pi_j}\}$
        \State $\pi_j' \leftarrow$ \textsc{FindPathAroundEnvelopes}($\calE_{\pi_j'}$)
        \If{success}
            \State \textsc{SetAvoidedEnvelopesOfPath($\pi_j', \calE_{\pi_j'}$)}
            \State $\Pi_{i+1} \leftarrow \Pi_{i+1} \cup \{\pi_j'\}$
        \Else
            \State $\Pi_{i+1} \leftarrow \Pi_{i+1} \cup \textsc{BisectAndFindMorePaths}(\calE_{\pi_j'})$ \label{alg1:bisect}
            % \State update $\calE_i$ in \calE
            % \State $\Pi \leftarrow \Pi \cup \Pi_{i+1}$
        \EndIf
    \EndFor
\EndFor
% \State \textbf{return} \Pi
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{\textsc{BisectAndFindMorePaths($\calE$)}} \label{alg2}
\AlgFontSize
\begin{algorithmic}[1]
    \State $\Pi \leftarrow \emptyset$
    % \State $\calE_\pi \leftarrow$ \textsc{GetAvoidedEnvelopesOfPath}($\pi$)
    % \State $\calE_\pi \leftarrow \calE_\pi \cup \{e\}$
    \State $e \leftarrow \calE$.pop()     \Comment{pop the best envelope to bisect}
    \If {\textsc{CheckSingleton}($e$)}    \Comment{contains one position}
        \State \textbf{return} $\emptyset$
    \EndIf
    \State $e^{l},e^{r} \leftarrow$ \textsc{BisectEnvelope($e$)}
    \State $\calE_{\pi_l} \leftarrow \calE \cup \{e^l\}$
    \State $\calE_{\pi_r} \leftarrow \calE \cup \{e^r\}$
    \For {each $\calE_{\pi_b} \in \calE_{\pi_l},\calE_{\pi_r}\}$}
    
        % first path
        % \State $\calE_{\pi_b} \leftarrow \calE \cup \{e^b\}$
        \State $\pi_b \leftarrow$ \textsc{FindPathAroundEnvelopes($\calE_{\pi_b}$)}
        \If{success}
            \State \textsc{SetAvoidedEnvelopesOfPath($\pi_b, \calE_{\pi_b}$)}
            \State $\Pi \leftarrow \Pi \cup \{\pi_b\}$
        \Else
            \State $\Pi \leftarrow \Pi \cup \textsc{BisectAndFindMorePaths}(\calE_{\pi_b})$
        \EndIf
    \EndFor
    % \State $\calE_s \leftarrow \calE_s \cup \{\tau_{a},\tau_{b}\}$
    \State \textbf{return} $\Pi$
    
    % \For {}
% \EndFor
\end{algorithmic}
\end{algorithm}
































\begin{comment}
\subsection{Theoretical Guarantees}
\subsubsection{Completeness}
Say we have access to a conventional motion planner $\calP$ in the preprocessing phase.
\begin{definition}[Strong]
Our algorithm is complete if it can find path to any $g \in G$ for any position of $o_M$ in $\calW$ within time bound $\Tbound$, provided $\calP$ can also find solution for the same problem in a large timeout $T_{\calP}$ 
\end{definition}
$$
OR
$$

\noindent Say we have access to a motion planner $\calP_{\rm DJ}$ in the preprocessing phase.
\begin{definition}[Weak]
Our algorithm is complete if it can find path to any $g \in G$ for any position of $o_M$ in $\calW$ within time bound $\Tbound$, provided $\calP_{\rm DJ}$ can find two disjoint paths for the same problem in a large timeout $T_{\calP_{\rm DJ}}$ 
\end{definition}

Also $\calP$ and $\calP_{\rm DJ}$ should be complete algorithms in the strict sense.

\subsection{Experience-based Planning}
Naive way would be to store a pair of disjoint paths ($\pi_a,\pi_b$) for each goal $g \in G$ where $G$ is the goal region for $o_T$ and then using lookup table $\calM: S \times G \rightarrow \{ (\pi^1_a, \pi^1_b), (\pi^2_a, \pi^2_b),... \}$ at query time to find the pair of paths for the given start $s$ and goal $g$.

Instead, we will use pairs of so called ``root paths" ($\Pi_a,\Pi_b$) (see~\cite{islam2020provably}) that will be used by an experience-based planner to reach sets of goals (within bounded time) instead of individual goals. In that case we will have the table $\calM: S \times G \rightarrow \{ (\Pi^1_a, \Pi^1_b), (\Pi^2_a, \Pi^2_b),... \}$. At query time, given $s,g$, we will lookup for ($\Pi_a,\Pi_b$) in $\calM$ and then use the experience-based planner (that will use ($\Pi_a,\Pi_b$)) to find the disjoint paths ($\pi_a,\pi_b$) from $s$ to $g$. 

\subsection{Implementation Details}
\subsubsection{Tunnel}
\begin{definition}
A tunnel around a path $\pi$ is defined as the volume spanned by an obstacle by placing it at all locations in its workspace, that intersect the path $\pi$.
\end{definition}

This is expensive to compute so we will use an approximation.

\subsubsection{Approximate Construction}
We will approximate the tunnel by a volume around the path defined by a radius $r$ where $r$ is related to the size of the obstacle. We pick some fixed points on the robot arm $\{p_1,p_2,...,p_k\}$.
Say the path $\pi$ has waypoints $\{q_{1},q_{2},...,q_{n}\}$.
A state $q$ of the robot would intersects the tunnel if $d_{\rm min} < r$ where $d_{\rm min}$ is the distance between the pair of closest points on $q$ and $\pi$.

    % \WHILE{!Success}
    %     \STATE $\{p_2, p_3,...\}, \{\tau_2, \tau_3,...\} \leftarrow $ \textsc{FindPathAroundEnvelope($p_1, \tau_1$)}
    %     \STATE 
        
    % \ENDWHILE

\newpage
\begin{algorithm}[t]
\caption{\textsc{PreprocessSingleObject()}}
\begin{algorithmic}[1]
    \STATE $p_1 \leftarrow$ \textsc{FindPathToGoal()}
    \STATE $\calP \leftarrow \{p_1\}$
    \STATE $e_1 \leftarrow$ \textsc{ConstructEnvelope($p_1$)}
    \STATE $p_2 \leftarrow$ \textsc{FindPathAroundEnvelope($e_{1}$)}
    \IF{success}
        \STATE  $\calP \leftarrow \calP \cup \{p_2\}$
    \ELSE
        \STATE $\calP \leftarrow \calP \cup \textsc{BisectEnvelopeAndFindMorePaths}(e_1)$
    \ENDIF
    \STATE \textbf{return} \calP 
    % \STATE $p_2, \leftarrow $ \textsc{FindPathAroundEnvelope($p_1, \tau_1$)}
    % \IF{fail}
    %     \STATE $\tau_{11},\tau_{12} \leftarrow$ \textsc{BisectEnvelope($\tau_1$)}
    %     \STATE \textsc{FindPathsAroundEnvelopes($\tau_{11},\tau_{12}$)}
    % \ENDIF
    % \STATE 
    
    % \FOR {}
% \ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{\textsc{BisectEnvelopeAndFindMorePaths($e$)}}
\begin{algorithmic}[1]
    \STATE $\calP \leftarrow \emptyset$
    \STATE $e_{a},e_{b} \leftarrow$ \textsc{BisectEnvelope($e$)}
    % first path
    \STATE $p_a \leftarrow$ \textsc{FindPathAroundEnvelope($e_{a}$)}
    \IF{success}
        \STATE $\calP \leftarrow \calP \cup \{p_a\}$
    \ELSE
        \STATE $\calP \leftarrow \calP \cup \textsc{BisectEnvelopeAndFindMorePaths}(e_{a})$
    \ENDIF
    \STATE Repeat for $e_b$
    \STATE \textbf{return} $\calP$
    
    % \FOR {}
% \ENDFOR
\end{algorithmic}
\end{algorithm}
\end{comment}


% \newpage

% \begin{algorithm}[t]
% \caption{\textsc{PreprocessMultipleObjects()}}
% \begin{algorithmic}[1]
% \STATE $p_0 \leftarrow$ \textsc{FindPathToGoal()}
% \STATE $\calP_0 \leftarrow p_0$
% \STATE $\calE \leftarrow \emptyset$
% \FOR{ i = 0 to N - 1 }
%     \STATE $\calE_i \leftarrow$ \textsc{ConstructEnvelopes($\calP_i$)}
%     \STATE $\calE \leftarrow \calE \cup \{\calE_i\}$
%     % \STATE $\calP_{i+1} \leftarrow$ 
%     \FOR{each $e \in \calE_i$}
%         \STATE $\calE_s \leftarrow$ \textsc{GetLinkedSetOfEnvelopes}($\calE,e$)
%         \STATE $p \leftarrow$ \textsc{FindPathAroundEnvelopes}($\calE_s$)
%         \IF{success}
%             \STATE $\calP_{i+1} \leftarrow \calP_{i+1} \cup \{p\}$
%         \ELSE
%             \STATE $\calP_{i+1} \leftarrow \calP_{i+1} \cup \textsc{BisectAnEnvelopeAndFindMorePaths}(\calE,e)$
%             % \STATE update $\calE_i$ in \calE
%             \STATE $\calP \leftarrow \calP \cup \calP_{i+1}$
%         \ENDIF
%     \ENDFOR
% \ENDFOR
% \STATE \textbf{return} \calP
% \end{algorithmic}
% \end{algorithm}




